Probabilistic Graphical Models for Credibility Analysis in Evolving Online Communities

One of the major hurdles preventing the full exploitation of information from online communities is the widespread concern regarding the quality and credibility of user-contributed content. Prior works in this domain operate on a static snapshot of the community, making strong assumptions about the structure of the data (e.g., relational tables), or consider only shallow features for text classification. To address the above limitations, we propose probabilistic graphical models that can leverage the joint interplay between multiple factors in online communities --- like user interactions, community dynamics, and textual content --- to automatically assess the credibility of user-contributed online content, and the expertise of users and their evolution with user-interpretable explanation. To this end, we devise new models based on Conditional Random Fields for different settings like incorporating partial expert knowledge for semi-supervised learning, and handling discrete labels as well as numeric ratings for fine-grained analysis. This enables applications such as extracting reliable side-effects of drugs from user-contributed posts in healthforums, and identifying credible content in news communities. Online communities are dynamic, as users join and leave, adapt to evolving trends, and mature over time. To capture this dynamics, we propose generative models based on Hidden Markov Model, Latent Dirichlet Allocation, and Brownian Motion to trace the continuous evolution of user expertise and their language model over time. This allows us to identify expert users and credible content jointly over time, improving state-of-the-art recommender systems by explicitly considering the maturity of users. This also enables applications such as identifying helpful product reviews, and detecting fake and anomalous reviews with limited information.

==> head/titlepage1.tex <==
\begin{titlepage}
\begin{center}
%\large
\sffamily


\null\vspace{2cm}
{\huge Probabilistic Graphical Models for Interpretable Credibility Analysis in Online Communities} \\[24pt]
%\textcolor{gray}{\small{THIS IS A TEMPORARY TITLE PAGE \\ It will be replaced for the final print by a version \\ provided by the service academique.}}
    
\vfill

\begin{tabular} {cc}
\parbox{0.3\textwidth}{\includegraphics[width=4cm]{images/epfl}}
&
\parbox{0.7\textwidth}{%
	Thèse n. 1234 2011\\
	présenté le 12 Mars 2011\\
	à la Faculté des Sciences de Base\\
	laboratoire SuperScience\\
	programme doctoral en SuperScience\\
%
%	ÉCOLE POLYTECHNIQUE FÉDÉRALE DE LAUSANNE\\
	École Polytechnique Fédérale de Lausanne\\[6pt]
	pour l'obtention du grade de Docteur ès Sciences\\
	par\\ [4pt]
	\null \hspace{3em} Subhabrata Mukherjee\\[9pt]
%
\small
acceptée sur proposition du jury:\\[4pt]
%
    Prof Name Surname, président du jury\\
    Prof Name Surname, directeur de thèse\\
    Prof Name Surname, rapporteur\\
    Prof Name Surname, rapporteur\\
    Prof Name Surname, rapporteur\\[12pt]
%
Lausanne, EPFL, 2011}
\end{tabular}
\end{center}
\vspace{2cm}
\end{titlepage}





==> main/chapter-credible-applications/consistency-analysis/conclusions.tex <==
\section{Conclusions}

We present a novel consistency model using limited information for detecting non-credible reviews which is shown to outperform state-of-the-art baselines. Our approach overcomes the limitation of existing works that make use of fine-grained information which are not available for ``long-tail'' items or newcomers in the community. Most importantly prior methods are not designed to {\em explain} why the detected review should be non-credible. In contrast, we make use of different {\em consistency features} from {\em latent facet model} derived from user text and ratings that can explain the assessments by our method. We develop multiple models for domain transfer and adaptation, where our model performs very well in the ranking tasks involving ``long-tail'' items, with as few as {\em five} reviews per-item.



==> main/chapter-credible-applications/consistency-analysis/introduction.tex <==
\section{Introduction}
\label{sec:intro}

%one par on problem and its importance
{\bf Motivation:} 
Online reviews about hotels, restaurants, consumer goods, movies, books, drugs, etc. are an invaluable resource for Internet users, providing a wealth of related information for potential 
customers. Unfortunately, corresponding forums such as TripAdvisor, Yelp, Amazon, and others are being increasingly game to manipulative and deceptive reviews: fake (to promote or demote some item), 
incompetent (rating an item based on irrelevant aspects), or biased (giving a distorted and inconsistent view of the item). For example, recent studies depict that $20\%$ of Yelp reviews might be 
fake and Yelp internally rejects $16\%$ of user submissions~\cite{Luca} as ``not-recommended''; with similar figures reported for reviews on Amazon.

Starting with the work of \cite{Liu2008}, research efforts have been undertaken to automatically detect non-credible reviews. In parallel, industry (e.g., stakeholders such as Yelp) has 
developed its own standards\footnote{\url{officialblog.yelp.com/2009/10/why-yelp-has-a-review-filter.html}} to filter out ``illegitimate'' reviews. Although details are not disclosed, studies suggest that these filters tend to be fairly 
crude~\cite{Liu2013a}; for instance, exploiting user activity like the number of reviews posted, and treating users whose ratings show high deviation from the mean/majority ratings as suspicious. Such a policy seems to 
over-emphasize trusted long-term contributors and suppress outlier opinions off the mainstream. Moreover, these filters also employ several aggregated metadata, and are thus hardly viable for 
new items that initially have very few reviews --- often by not so active users or newcomers in the community.

%state-of-the-art research methods and their limitations
\noindent {\bf State of the Art:}
Research on this topic has cast the problem of review credibility into a binary classification task: a review is either credible or deceptive.
To this end, supervised and semi-supervised methods have been developed that largely rely on features about users and their activities as well as statistics about item ratings. 
Most techniques also consider spatio-temporal patterns of user activities like 
IP addresses or user locations (e.g., \cite{Liu2014,Li2015}), 
burstiness of posts on an item or an item group (e.g., \cite{Fei2013}), 
and further 
correlation measures across users and items (e.g., \cite{mukherjee2014peopleondrugs}). 
However, the classifiers built this way are mostly geared for popular items, and the meta-information about user histories and activity correlations are not always available. For example, 
someone interested in opinions on a new art film or a ``long-tail'' bed-and-breakfast in a rarely visited town, is not helped at all by the above methods. 
%for review credibility classification.
%
%now one short par on text-based approaches
Several existing works~\cite{Mihalcea2009,Ott2011,Ott2013} consider the textual content of user reviews for tackling opinion spam by using word-level unigrams or bigrams as features, 
along with specific lexicons (e.g., LIWC~\cite{liwc} psycholinguistic lexicon, WordNet Affect~\cite{wordnetaffect}), to learn latent topic models and classifiers (e.g., \cite{Ott2013a}).
%
Although these methods achieve high classification accuracy for various gold-standard datasets, they do not provide any interpretable evidence as to why a certain review is classified as 
non-credible.


\noindent {\bf Problem Statement:}
This paper focuses on detecting credible reviews {\em with limited information}, namely, in the absence of rich data about user histories, community-wide correlations, and for ``long-tail'' items. 
In the extreme case, we are provided with only the review texts and ratings for an item. Our goal is then to compute a {\em credibility score} for the reviews and to provide possibly 
{\em interpretable evidence} for explaining why certain reviews have been categorized as non-credible.
 

\noindent {\bf Approach:}
Our proposed method to this end is to learn a model based on {\em latent topic models} and combining them with limited metadata to provide a novel notion of {\em consistency features} 
characterizing each review. We use the LDA-based Joint Sentiment Topic model (JST)~\cite{Lin2009} to cast the user review texts into a number of informative facets. We do this per-item, 
aggregating the text among all reviews for the same item, and also per-review. This allows us to identify, score, and highlight inconsistencies that may appear between a review and 
the community's overall characterization of an item. We perform this for the item as a whole, and also for each of the latent facets separately.
Additionally, we learn inconsistencies such as discrepancy between the contents of a review and its rating, and temporal ``bursts'' --- where a number of reviews are written in a short span 
of time targeting an item. We propose five kinds of inconsistencies that form the key assets of our credibility scoring model, fed into a Support Vector Machine for classification, or for ordinal ranking.


\noindent {\bf Contribution:} In summary, our contributions are summarized as:
\squishlist
 \item {\em Model:} We develop a novel {\em consistency model} for credibility analysis of reviews that works with limited information, with particular attention to ``long-tail'' items, and offers interpretable evidence for reviews classified as non-credible.
 \item {\em Tasks:} We investigate how credibility scores affect the overall ranking of items. To address the scarcity of labeled training data, we transfer the learned model from Yelp to Amazon to rank top-selling items based on (classified) {\em credible} user reviews. In the presence of proxy labels for item ``goodness'' (e.g., item sales rank), we develop a better ranking model for domain adaptation.% in the community.
 \item {\em Experiments:} We perform extensive experiments in TripAdvisor, Yelp, and Amazon to demonstrate the viability of our method and its advantages over state-of-the-art baselines in dealing with ``long-tail'' items and providing interpretable evidence.
\squishend

%%%%%%%%%%
%%%GW: old text follow, commented out
\begin{comment}
In this work, we want to perform {\em credibility analysis} of reviews where we want to find the most relevant reviews on an item.
%analyzing different facets of an item. 
An important component of this task is the {\em consistency analysis} of reviews, where we want to exploit inconsistencies in user ratings, review text, and facet description. This way we can give some interpretations as to why we consider a review as non-credible. This is an important distinction between our work and previous works in this domain.

Previous works in fake review detection, and opinion spam detection primarily focused on two different aspects of the problem: 

\noindent {\bf Linguistic Analysis}~\cite{Mihalcea2009,Ott2011,Ott2013} --- The authors exploit the distributional difference in the wordings of authentic and manually-created fake reviews using word-level features. However, the artificially created fake review dataset for the given task give away some explicit features that are not dominant in real-world data. This was confirmed by a study on Yelp filtered reviews~\cite{Liu2013a} where these $n$-gram features performed very poorly despite their outstanding performance on the Amazon Mechanical Turk generated fake review dataset.

\noindent {\bf Rating and Activity Analysis} --- In absence of ground-truth data, prior works make simplistic assumptions, e.g. duplicates and near-duplicates are fake~\cite{Liu2007,Liu2008,Liu2010,Liu2011,Liu2012,Liu2013,Liu2013a,Liu2014,Rahman2015}, and make use of background information like brand name, item description, user session history etc. Thereafter, they train regression models using several features derived from : a) extreme ratings, b) user activity (number of posts, friends etc.), c) review length d) rating deviation from community mean, e) burstiness, and f) simple language features like content similarity, presence of literals, numerals, capitalizations, and POS tags. 

The primary issue with these works is that they either make use of very fine-grained information which are difficult to obtain for different communities, and hence cannot be generalized; and most importantly do not {\em explain} why the detected review should be fake. In contrast, we make use of different {\em consistency features} derived only from the user text and ratings that can be used to explain some of these observations, and can be generalized without the requirement of additional information. 
\end{comment}
%%%%%%%%%%%%





==> main/chapter-credible-applications/consistency-analysis/related-work.tex <==
\section{Related Work}

Previous works in fake review and opinion spam detection primarily focused on two different aspects of the problem: 

\noindent {\bf Linguistic Analysis}~\cite{Mihalcea2009,Ott2011,Ott2013} -- This approach exploits the distributional difference in the wordings of authentic and manually-created 
fake reviews using word-level features. However, artificially created fake review datasets for the studied tasks give away explicit features not dominant in 
real-world data. This was confirmed by a study on Yelp filtered reviews~\cite{Liu2013a}, where the $n$-gram features performed poorly despite their outstanding performance 
on the Amazon Mechanical Turk generated fake review dataset. Additionally, linguistic features such as {\em text sentiment}~\cite{Yoo2009}, {\em readability score} 
(e.g., Automated readability index (ARI), Flesch reading ease, etc.)~\cite{Hu2012}, {\em textual coherence}~\cite{Mihalcea2009}, and rules based on 
{\em Probabilistic Context Free Grammar} (PCFG)~\cite{Feng2012} have been studied.

\noindent {\bf Rating and Activity Analysis} -- In the absence of proper ground-truth data, prior works make simplistic assumptions, e.g., duplicates and near-duplicates are 
fake, and make use of {\em extensive} background information like brand name, item description, user history, IP addresses and location, etc.~\cite{Liu2007,Liu2008,Liu2010,Liu2011,Liu2012,Liu2013,Liu2013a,Liu2014,Rahman2015}. 
Thereafter, regression models trained on all these features are used to classify reviews as credible or deceptive. Some of these works also use crude or ad-hoc language 
features like content similarity, presence of literals, numerals, and capitalization.
%
In contrast to these works, our approach uses limited information about users and items catering to a broad domain of applications. We harvest several consistency features from user 
rating and review text that give some interpretation as to why a review should be deemed non-credible.

\noindent {\bf Learning to Rank} -- Supervised models have also been developed to rank items from constructed item feature vectors~\cite{liu2009}. Such techniques optimize measures like Discounted Cumulative Gain, Kendall-Tau, and Reciprocal Rank to generate item ranking similar to the training data based on the feature vectors. We use one such technique, and show its performance can be improved by removing non-credible item reviews.
%As such, a related area of study involves 
%the re-ranking of items according to their proper rating, wherein the ``credible'' reviews are implicitly gauged based on the feature vectors.



==> main/chapter-credible-applications/helpful-reviews/conclusion.tex <==

\section{Conclusion}\label{sec:conc}

In this paper, we propose an approach to predict review helpfulness by exploiting the {\em joint interaction} between user expertise, writing style, timeliness, and review consistency using Hidden Markov Model -- Latent Dirichlet Allocation. Unlike prior works exploiting a variety of syntactic and domain-specific features, our model uses {\em only} the information of a user reviewing an item at an explicit timepoint to perform this task --- making our approach generalizable across all communities and domains. Additionally, we provide {\em interpretable explanation} as to why a review is helpful, in terms of salient words from latent word clusters --- that are used by experts to describe important facets of the item under consideration.

We perform extensive experiments on real-world reviews from different domains in Amazon like books, movies, music, food, and electronics, that demonstrate the effectiveness of our approach over state-of-the-art baselines.

%Current recommender systems do not consider user experience when generating recommendations. 
%In this paper, 
%we have proposed an experience-aware recommendation model that can adapt to the changing preferences and maturity of users in a community.
%%
%We model the {\em personal evolution} of a user in rating items that she will appreciate at her current maturity level. 
%We exploit the coupling between the \emph{facet preferences} of a user, her \emph{experience}, \emph{writing style} in reviews, and \emph{rating behavior} to capture the user's temporal evolution.
%Our model is the first work that considers the progression of user experience as expressed in the text of item reviews.

%We propose a generative HMM-LDA model for tracing a user's evolution, where %the Hidden Markov Model (HMM) traces her latent experience progressing over %time, and the Latent Dirichlet Allocation (LDA) model captures her interest %in specific item facets as a function of her (again latent) experience level %and writing style. The model considers user assigned ratings to items and 
%review text till a given timepoint as observables, and outputs the rating 
%the user would assign to an item at a later timepoint based on her evolved 
%experience.

%Our experiments -- with data from domains like beer, movies, food, and news -- demonstrate that our model substantially reduces the mean squared error for predicted ratings, compared to the state-of-the-art baselines. 
%This shows our method can generate better recommendations than those models.
%We further demonstrate the utility of our method in a use-case study about identifying experienced members in the NewsTrust community who can be potential citizen journalists.

%Overall in this work we propose an experience-aware recommendation model 
%that can adapt to the changing preferences and maturity of users in a community.

==> main/chapter-credible-applications/helpful-reviews/introduction.tex <==

\section{Introduction}

\noindent {\bf Motivation:} With the rapid growth in e-Commerce, product reviews have become a crucial component for the business in recent times. As consumers cannot test the functionality of a product prior to purchase, these reviews help them make an informed decision to buy the product or not. As per the survey conducted by Nielsen Corporations, $40\%$ of online consumers have indicated that they would not buy electronics without consulting online reviews first~\cite{nielsen}. 

Due to the increasing dependency on user-generated reviews, it is crucial to understand their quality --- that can widely vary from being an excellent-detailed opinion to superficial criticizing or praising, to spams in the worst case. Without any indication of the review quality, it is overwhelming for consumers to browse through a multitude of reviews. In order to help consumers in finding useful reviews, most of the e-Commerce platforms nowadays allow users to vote whether a product review is helpful or not. For instance, any {\em Amazon} product review is accompanied with information like $x$ out of $y$ users found the review helpful. This {\em helpfulness score} ($x/y$) can be considered as a proxy for the review quality. In this work, we aim to automatically find the helpfulness score of a review based on certain consistency, and semantic aspects of the review like: whether the review is written by an expert, what are the important facets of the product outlined in his review, what do other 
experts have to say about the given product, timeliness of the review etc.

%These external votes about the review helpfulness assist new consumers in focusing on the helpful reviews. 
%In this work, we aim to determine the helpfulness +of a review based on various semantic aspects.\\

\noindent {\bf State-of-the-Art and its Limitations:} Prior works on predicting review helpfulness mostly operate on shallow syntactic textual features like bag-of-words, part-of-speech tags, and tf-idf (term, and inverse document frequency) statistics~\cite{Kim:2006:AAR:1610075.1610135,Lu:2010:ESC:1772690.1772761}. These works, and other related works on finding review spams~\cite{Liu2008, Liu2013} classify extremely opinionated reviews as not helpful. Similarly, other works exploiting rating \& activity features like frequency of user posts, average ratings of users and items~\cite{O'Mahony:2009:LRH:1639714.1639774,Lu:2010:ESC:1772690.1772761, liu-EtAl:2007:EMNLP-CoNLL2007} consider extreme ratings and deviations as indicative of unhelpful reviews. Some recent works incorporate additional information like community-specific characteristics (who-voted-whom) with explicit user network~\cite{Tang:2013:CRH:2507157.2507183,Lu:2010:ESC:1772690.1772761}, and item-specific meta-data like {\em explicit} item facets 
and product brands~\cite{icdm2008,Kim:2006:AAR:1610075.1610135}. Apart from the requirement of a large number of meta-features that restrict the generalizability of many of these models to any arbitrary domain, these shallow features do not 
analyze what the review is {\em about}, and, therefore, cannot {\em explain} why it should be helpful for a given product. Some of these works~\cite{O'Mahony:2009:LRH:1639714.1639774,icdm2008} identify {\em expertise} of a review's author as an important feature. However, in absence of suitable modeling techniques, they consider prior reputation features like user activity, and low rating deviation as proxy for user expertise. 

The work closest to our approach is~\cite{icdm2008} --- where the authors identify syntactic features, user expertise, and timeliness of a review as important indicators of its quality. However, even in this case, the authors use part-of-speech tags as syntactic features, and user preferences for {\em explicit} item facets (pre-defined genres of IMDB movies in their work) as proxy for user expertise. In contrast, we explicitly model user expertise as a function of their writing style, rating style, and preferences for (latent) item facets --- all of which are jointly learned from user-generated reviews --- going beyond the usage of shallow syntactic features, and the requirement for additional item meta-data.

\noindent {\bf Problem:} Our work aims to overcome the limitations of prior works by exploring the {\em semantics} and {\em consistency} of a review to predict its {\em helpfulness score} for a given item. Unlike prior works, all of these features can be harnessed from only the information of a {\em user reviewing an item at an explicit timepoint}, making our approach fairly general for all communities and domains. We also provide {\em interpretable} explanation in terms of latent word clusters that gives interesting insights as to what makes the review helpful.\\
%\noindent {\bf Example:}\\
\noindent {\bf Approach:} The first step towards understanding the {\em semantics} of a review is to uncover the facet descriptions of the target item outlined in the review. We treat these facets as {\em latent} and use Latent Dirichlet Allocation (LDA) to discover them as topic clusters. The second step is to find the {\em expertise} of the users who wrote the review, and their description of the different (latent) facets of the item. User expertise has been modeled only recently~\cite{mcauleyWWW2013,mukherjee2015jertm} for recommender systems. In this work, we model expertise as a {\em latent} variable that evolves over time using a Hidden Markov Model (HMM), 
%similar to~\cite{mukherjee2015jertm}, 
but with significant differences and modifications (outlined in Section~\ref{subsec:diff}) over the prior works --- especially for modeling the joint interaction between several factors, where our proposed model has a better coupling between the factors, all of which are learned directly from the review helpfulness.

We make use of {\em distributional hypotheses} (outlined in Section~\ref{subsec:distrhyp}) like: expert users agree on what are the important facets of an item, and their description (or, writing style) of those facets 
influences the helpfulness of a review. We also derive several {\em consistency} 
features --- all from the given quintuple $\langle$\textit{userId, itemId, rating, reviewText, timepoint}$\rangle$ --- like prior user reputation, item prominence, and timeliness of a review, that are used in conjunction with the semantic features. Finally, we leverage the interplay between all of the above factors in a {\em joint} setting to predict the review helpfulness.

For interpretable explanation, we derive interesting insights from the latent word clusters used by experts --- for instance, reviews describing the underlying ``theme and storytelling'' of {\em movies} and {\em books}, the ``style'' of {\em music}, and ``hygiene'' of {\em food} are considered most helpful for the respective domains.

\noindent The salient contributions of this paper can be summarized as:

\squishlisttwo
\item[a)] {\bf Model:} We propose an approach to leverage the {\em semantics} and {\em consistency} of reviews to predict their helpfulness. We propose a Hidden Markov Model -- Latent Dirichlet Allocation (HMM-LDA) based model that jointly learns the (latent) item facets, (latent) user expertise, and his writing style from {\em observed} words in reviews at explicit timepoints. 
\item[b)] {\bf Algorithm:} We introduce an effective learning algorithm based on an iterative stochastic optimization process that reduces the mean squared error of the predicted helpfulness scores with the ground scores, as well as maximizes the log-likelihood of the data.
\item[c)] {\bf Experiments:} We perform large-scale experiments with real-world datasets from {\em five} different domains in {\em Amazon}, together comprising of $29$ million reviews from $5.7$ million users on $1.9$ million items, and demonstrate substantial improvement over state-of-the art baselines for {\em prediction} and {\em ranking} tasks.
\squishend

\noindent The rest of the paper is organized as follows: Section~\ref{sec:features} introduces the different semantic and consistency factors to model review helpfulness, along with a preliminary study. Section~\ref{sec:model} presents the HMM-LDA based model to {\em jointly} infer the item facets, user expertise, and review helpfulness, along with an inference method based on Gibbs sampling and regression. Section~\ref{sec:experiments} presents the experimental evaluation of our approach, comparing it against several baselines, followed by related works and conclusion in Section~\ref{sec:relWork} and Section~\ref{sec:conc}, respectively.




==> main/chapter-credible-applications/helpful-reviews/relatedwork.tex <==
\section{Related Work}\label{sec:relWork}

Prior works on predicting review helpfulness~\cite{Kim:2006:AAR:1610075.1610135,Lu:2010:ESC:1772690.1772761} exploit shallow syntactic features to classify extremely opinionated reviews as not helpful. Similar features are also used in finding review spams~\cite{Liu2008, Liu2013}. Similarly, few other approaches utilize features like frequency of user posts, average ratings of users and items to distinguish between helpful and unhelpful reviews. Community-specific features with explicit user network are used in~\cite{Tang:2013:CRH:2507157.2507183,Lu:2010:ESC:1772690.1772761}. However, these shallow features do not analyze what the review is {\em about}, and, therefore, cannot {\em explain} why it should be helpful for a given product. 

Approaches proposed in~\cite{icdm2008,Kim:2006:AAR:1610075.1610135} also utilize item-specific meta-data like {\em explicit} item facets and product brands to decide the helpfulness of a review. However, these approaches heavily rely on a large number of meta-features which makes them less generalizable. Some of the related approaches~\cite{O'Mahony:2009:LRH:1639714.1639774,icdm2008} also identify {\em expertise} of a review's author as an important feature. However, they do not explicitly model the user expertise. 

Recent work in \cite{mcauleyWWW2013} studies the influence of rating behavior on evolving user experience. However, it does not consider the vocabulary and writing style of users in reviews, and their temporal progression. 
%In contrast, our work gains additional insights by considering the review texts to capture the facet preferences and experience progression. 
Our model for capturing user expertise draws motivation from~\cite{mukherjee2015jertm},\cite{mcauleyWWW2013} with significant differences. Unlike prior works, the facet preferences in our model is conditioned only on the user expertise and not the user. This significantly reduces the dimensionality of the model making it more efficient; as well as the distributions are learned directly from minimizing the mean squared error for predictions, allowing all parameters to be coupled tightly, unlike in~\cite{mukherjee2015jertm}.

User review text is also considered in Sentiment Analysis. These approaches aim to learns latent topics~\cite{linCIKM2009}, latent aspects and their ratings~\cite{lakkarajuSDM2011,wang2011,mcauleyrecsys2013}, and user-user interactions~\cite{West-etal:2014}. The author writing style is also used in \cite{mukherjeeSDM2014}. However, all of these prior approaches do not consider time or user expertise to capture the evolving writing style.

==> main/chapter-temporal-evolution/cont-model/conclusion.tex <==
\vspace*{-1mm}\section{Conclusion}
In this paper,
we have proposed an experience-aware language model that can trace the {\em continuous} evolution of user experience and language explicitly over {\em time}.
%
We combine principles of Geometric Brownian Motion, Brownian Motion, and Latent Dirichlet Allocation to model a smooth temporal progression of user experience, and language model over time.
This is the first work to develop a continuous and generalized version of user experience evolution.

%We propose a generative HMM-LDA model for tracing a user's evolution, where %the Hidden Markov Model (HMM) traces her latent experience progressing over %time, and the Latent Dirichlet Allocation (LDA) model captures her interest %in specific item facets as a function of her (again latent) experience level %and writing style. The model considers user assigned ratings to items and 
%review text till a given timepoint as observables, and outputs the rating 
%the user would assign to an item at a later timepoint based on her evolved 
%experience.

Our experiments -- with data from domains like beer, movies, food, and news -- demonstrate that our model effectively exploits user experience for item recommendation that
substantially reduces the mean squared error for predicted ratings, compared to the state-of-the-art baselines~\cite{mcauleyWWW2013,Subho:ICDM2015}. 

We further demonstrate the utility of our model in a use-case study about identifying experienced members in the NewsTrust community, where these users would be top candidates for being citizen journalists. Another similar use-case for our model can be to detect experienced medical professionals in the health community.% who can contribute valuable medical knowledge.

%Overall in this work we propose an experience-aware recommendation model 
%that can adapt to the changing preferences and maturity of users in a community.

==> main/chapter-temporal-evolution/cont-model/relatedwork.tex <==
\section{Related Work}

%%%GW: re-worded the following paragraph, to make it look different from the ICDM paper
State-of-the-art recommender systems \cite{korenKDD2008, koren2011advances} 
harness user-user and item-item similarities by means of latent factor models. 
Time-dependent phenomena such as bursts in item popularity, bias in ratings, 
and the temporal evolution of user community are investigated in~\cite{KorenKDD2010, xiongSDM2010, XiangKDD2010}. There is also prior work on anomaly detection~\cite{GunnemannGF14,Gunnemann2014}, capturing changes of social links~\cite{MaWSDM2011} and linguistic norms~\cite{DanescuWWW2013}. 
None of these prior works take into account the evolving experience and behavior of individual users.

Prior work that analyzed user review texts focused on sentiment analysis~\cite{linCIKM2009}, learning latent aspects and their ratings~\cite{wang2011, mukherjeeSDM2014, mcauleyRecSys2013}, and user-user interactions~\cite{West-etal:2014}. 
However, all of these prior approaches operate in a static, snapshot-oriented manner, without considering time at all.

The work~\cite{mcauleyWWW2013}, one of our baselines, has modeled and studied the influence of evolving user experience on rating behavior and for targeted recommendations. However, it disregards the vocabulary in the users' reviews. 
Our own recent work~\cite{Subho:ICDM2015} addressed this very limitation,
by means of language models that are specific to the experience level of an
individual user, and by modeling transitions between experience levels with a Hidden
Markov Model.
However, both of these works are limited to {\em discrete} experience levels leading to abrupt changes in both experience and language model. To address the above, and other related drawbacks, the current paper introduces continuous-time models for the smooth evolution of both
user experience and language model.


%%%GW: added one par on dynamic topic models
Wang et al.~\cite{Wang2006} modeled topics over time. However, the topics
themselves were constant, and time was only
used to better discover them. Dynamic topic models have been introduced by Blei et al. in 
\cite{BleiDTM,BleiCTM}. This prior work developed generic models
based on Brownian Motion, and applied them
to news corpora. 
\cite{BleiCTM} argues that the continuous model
avoids making choices for discretization and is also
more tractable compared to fine-grained discretization.
Our language model is motivated by the latter. We substantially extend it to capture evolving user behavior and experience
in review communities using Geometric Brownian Motion.
%\cite{BleiCTM} presents variational inference techniques, 
%whereas our work adopts Metropolis-Hastings
%sampling.



%%%GW: I believe the following can be dropped
%%% in the case it is revived, it needs to be re-worded a bit, to make the wording differ from the ICDM paper
%
%From the modeling perspective, some approaches learn a document-specific discrete %rating~\cite{linCIKM2009, ramageKDD2011}, whereas others learn the facet weights outside the %topic model~\cite{lakkarajuSDM2011, mcauleyRecSys2013, mukherjeeSDM2014}. In order to %incorporate continuous ratings,~\cite{bleiNIPS2007} proposed a complex and computationally %expensive Variational Inference algorithm, and~\cite{mimnoUAI2008} developed a simpler %approach using Multinomial-Dirichlet Regression. 


==> main/chapter-temporal-evolution/cont-model/usecases.tex <==

\subsection{Use-Case Study}
\label{sec:usecases}

So far we have focused on traditional item recommendation for items like beers or movies. Now we switch to different kind of items - newspapers and news articles - by analyzing the NewsTrust online community ({\tt \href{http://www.newstrust.net}{newstrust.net}})~\footnote{Data available at \url{http://www.mpi-inf.mpg.de/impact/credibilityanalysis/}.}. It features news stories posted and reviewed by members, 
%many
some of whom are professional journalists and content experts. Stories are reviewed based on their objectivity, rationality, and general quality of language to present an unbiased and balanced narrative of an event with focus on \emph{quality journalism}. Unlike the other datasets, NewsTrust contains expertise of members that can be used as ground-truth for evaluating our model-generated {\em experience} values.

In our framework, each story is an item, which is rated and reviewed by a user. The facets are the underlying topic distribution of the reviews, with topics being {\em Healthcare, Obama Administration, NSA}, etc. The facet preferences can be mapped to the (political) polarity of users in this news community. 

\subsubsection{Recommending News Articles}

Our first objective is to recommend news to readers catering to their viewpoints, and experience. We apply our model with the same setting as with earlier datasets.
%We apply our model to this task, and compare the predicted ratings with the ones observed for withheld reviews in the NewsTrust community. 
The mean squared error (MSE) results were reported in Section~\ref{sec:experiments}. Our model clearly outperforms most of the baselines; it performs only slightly worse regarding our prior discrete model (discussed in Section~\ref{sec:discrete}) in this task --- possibly due to high rating sparsity in face of a large number of model parameters. 

%Although our model outperforms most of the baselines, it performs a bit worse than the discrete model (our prior work~\cite{Subho:ICDM2015}) in this task.

%One reason can be due to less data available per-user in this community to learn long-term experience evolution.
%Table~\ref{tab:newstrustTopics} shows salient examples of the vocabulary by users at different experience levels on the topic {\em US Election}. As one can see, the language of users from different experience levels varies greatly, confirming the need for experience aware facet models.


%\paragraph{Identifying Experienced Users}

\subsubsection{Identifying Experienced Users}

Our second task is to find experienced members of this community, who have the potential of being \emph{citizen journalists}. In order to evaluate the quality of the ranked list of experienced users generated by our model, we consider the following proxy measure for user experience. In NewsTrust, users have {\em Member Levels} determined by the NewsTrust staff based on  community engagement, time in the community, other users' feedback on reviews, profile transparency, and manual validation.
We use these member levels to categorize users as {\em experienced} or {\em inexperienced}. This is treated as the ground truth for assessing the ranking quality of our model against the baseline models~\cite{mcauleyWWW2013}, and the discrete version of our prior work (discussed in Section~\ref{sec:discrete}) --- considering top $100$ users from each model ranked by experience. Here we consider the top-performing baseline models from the previous task.
%\todo{this is a bit unclear; we rank our users according to experience. and then? we use top k? how many?}
%Table~\ref{tab:ndcgUsers} shows the $F_1$ scores of these two competitors.
We report the \emph{Normalized Discounted Cumulative Gain (NDCG)} % \cite{Jarvelin:TOIS2002} 
and the {\em Normalized Kendall Tau Distance} 
%Kalervo Jarvelin, Jaana Kekalainen: Cumulated gain-based evaluation of IR 
%techniques. ACM Transactions on Information Systems 20(4), 422–446 (2002)
for the ranked lists of users generated by all the models. The better model should exhibit higher {\em NDCG}, and lower {\em Kendall Tau Distance}. 
As Table~\ref{tab:ndcgUsers} shows, our model outperforms baseline models in capturing user maturity.

\comment{
NDCG gives geometrically decreasing weights to predictions at the various positions of the ranked list:

{\small
$NDCG_p = \frac{DCG_p}{IDCG_p}$ where
$DCG_p = rel_1 + \sum_{i=2}^p \frac{rel_i}{\log_2 i}$
}

Here, $rel_i$ is the relevance ($0$ or $1$) of a result at position $i$. 
%DCG penalizes relevant items (\emph{experienced users}) appearing lower in 
%the rank list, where the graded relevance score is reduced logarithmically 
%proportional to the position of the result. 
%As the length of lists may vary for different queries, DCG scores are 
%normalized using the ideal score, IDCG where the results of a rank list are 
%sorted by relevance giving the maximum possible DCG score.
}

%We also report the {\em Normalized Kendall Tau Distance} of the ranked lists given by the models, against the ground truth rank list.

\begin{table}
\begin{center}
%\centering
 \setlength{\tabcolsep}{2mm}
 \begin{tabular}{p{6cm}p{2cm}p{4cm}}
 \toprule
\bf{Models} &\bf{NDCG} & \bf{Kendall Tau}\\
\bf{} & \bf{} & \bf{Normalized Distance}\\
\midrule 
{\bf Continuous experience model}\newline (this work) & {\bf 0.917} & {\bf 0.113} \\
Discrete experience model\newline (refer to Section~\ref{sec:discrete}) & 0.898 & 0.134 \\
User at learned rate~\cite{mcauleyWWW2013} & 0.872 & 0.180 \\
\bottomrule
 \end{tabular}
\caption{\hspace{0.3em}Performance on identifying experienced users.}
\label{tab:ndcgUsers}
\end{center}
\end{table}


==> main/chapter-temporal-evolution/discrete-model/conclusion.tex <==

\section{Conclusion}

Current recommender systems do not consider user experience when generating recommendations. 
In this paper, 
we have proposed an experience-aware recommendation model that can adapt to the changing preferences and maturity of users in a community.
%
We model the {\em personal evolution} of a user in rating items that she will appreciate at her current maturity level. 
We exploit the coupling between the \emph{facet preferences} of a user, her \emph{experience}, \emph{writing style} in reviews, and \emph{rating behavior} to capture the user's temporal evolution.
Our model is the first work that considers the progression of user experience as expressed in the text of item reviews.

%We propose a generative HMM-LDA model for tracing a user's evolution, where %the Hidden Markov Model (HMM) traces her latent experience progressing over %time, and the Latent Dirichlet Allocation (LDA) model captures her interest %in specific item facets as a function of her (again latent) experience level %and writing style. The model considers user assigned ratings to items and 
%review text till a given timepoint as observables, and outputs the rating 
%the user would assign to an item at a later timepoint based on her evolved 
%experience.

Our experiments -- with data from domains like beer, movies, food, and news -- demonstrate that our model substantially reduces the mean squared error for predicted ratings, compared to the state-of-the-art baselines. 
This shows our method can generate better recommendations than those models.
We further demonstrate the utility of our method in a use-case study about identifying experienced members in the NewsTrust community who can be potential citizen journalists.

%Overall in this work we propose an experience-aware recommendation model 
%that can adapt to the changing preferences and maturity of users in a community.

==> main/chapter-temporal-evolution/discrete-model/relatedwork.tex <==
\section{Related Work}

State-of-the-art recommenders based on collaborative filtering \cite{korenKDD2008}\cite{koren2011advances} exploit user-user and item-item similarities by latent factors. Explicit user-user interactions have been exploited in trust-aware recommendation systems~\cite{GuhaWWW2004}\cite{West-etal:2014}. The temporal aspects leading to bursts in item popularity, bias in ratings, or the evolution of the entire community as a whole is studied in~\cite{KorenKDD2010}\cite{xiongSDM2010}\cite{XiangKDD2010}. Other papers have studied temporal issues for anomaly detection~\cite{Gunnemann2014}, detecting changes in the social neighborhood~\cite{MaWSDM2011} and linguistic norms~\cite{DanescuWWW2013}. However, none of these prior work has considered the evolving experience and behavior of individual users.

The recent work\cite{mcauleyWWW2013}, which is one of our baselines, modeled the influence of rating behavior on evolving user experience. However, it ignores the vocabulary and writing style of users in reviews, and their natural {\em smooth} temporal progression. In contrast, our work considers the review texts for additional insight into facet preferences and {\em smooth} experience progression.

Prior work that tapped user review texts focused on other issues. Sentiment analysis over reviews aimed to learn latent topics~\cite{linCIKM2009}, latent aspects and their ratings~\cite{lakkarajuSDM2011}\cite{wang2011}, and user-user interactions~\cite{West-etal:2014}. \cite{mcauleyRecSys2013}\cite{WangKDD2011} unified various approaches to generate user-specific ratings of reviews. \cite{mukherjeeSDM2014} further leveraged the author writing style. However, all of these prior approaches operate in a static, snapshot-oriented manner, without considering time at all.

From the modeling perspective, some approaches learn a document-specific discrete rating~\cite{linCIKM2009}\cite{ramageKDD2011}, whereas others learn the facet weights outside the topic model (e.g., ~\cite{lakkarajuSDM2011, mcauleyRecSys2013, mukherjeeSDM2014}). In order to incorporate continuous ratings,~\cite{bleiNIPS2007} proposed a complex and computationally expensive Variational Inference algorithm, and~\cite{mimnoUAI2008} developed a simpler approach using Multinomial-Dirichlet Regression. The latter inspired our technique for incorporating supervision.
%GW: is the last sentence - "inspired ..." - adequate?

==> main/chapter-temporal-evolution/discrete-model/usecases.tex <==

\subsection{Use-Case Study}
\label{sec:usecases}

So far we have focused on traditional item recommendation for items like beers or movies. Now we switch to a different kind of items - newspapers and news articles - tapping into the NewsTrust online community ({\tt \href{www.newstust.net}{newstrust.net}}). NewsTrust features news stories posted and reviewed by members, 
many of whom are professional journalists and content experts. Stories are reviewed based on their objectivity, rationality, and general quality of language to present an unbiased and balanced narrative of an event. The focus is on \emph{quality journalism}. Previously in Section~\ref{sec:newstrust-data}, we discussed several characteristics of this community that were employed for credibility analysis therein.

In our framework of item recommendation, each story is an item, which is rated and reviewed by a user. The facets are the underlying topic distribution of reviews, with topics being {\em Healthcare, Obama Administration, NSA}, etc. The facet preferences can be mapped to the (political) polarity of users in the news community. 

\subsubsection{Recommending News Articles}

Our first objective is to recommend news to readers catering to their facet preferences, viewpoints, and experience. We apply our joint model to this task, and compare the predicted ratings with the ones observed for withheld reviews in the NewsTrust community. The mean squared error (MSE) results are reported in Table~\ref{fig:MSE1} in Section~\ref{sec:experiments1}. Table~\ref{tab:newstrustTopics} shows salient examples of the vocabulary by users at different experience levels on the topic {\em US Election}.

\begin{table}
\small
\centering
\begin{tabular}{p{12cm}}
\toprule
\textbf{Level 1:} bad god religion iraq responsibility\\
\textbf{Level 2:} national reform live krugman questions clear jon led meaningful lives california powerful safety impacts\\
\textbf{Level 3:} health actions cuts medicare nov news points oil climate major jobs house high vote congressional spending unemployment strong taxes citizens events failure\\
\bottomrule
\end{tabular}
\caption{Salient words for the {\em illustrative} NewsTrust topic {\em US Election} used by users at different levels of experience.}
\label{tab:newstrustTopics}
\end{table}

%\paragraph{Identifying Experienced Users}

\begin{table}
\begin{center}
 \begin{tabular}{lcc}
 \toprule
\bf{Models} & \bf{$F_1$} & \bf{$NDCG$}\\
\midrule
User at learned rate~\cite{mcauleyWWW2013} & 0.68 & 0.90 \\
Our model & 0.75 & 0.97 \\
\bottomrule
 \end{tabular}
\caption{Performance on identifying experienced users.}
\label{tab:ndcgUsers}
\end{center}
\end{table}

\subsubsection{Identifying Experienced Users}

Our second task is to find experienced members of this community, who have potential for being \emph{citizen journalists}. In order to find how good our model predicts the experience level of users, we consider the following as ground-truth for user experience. In NewsTrust, users have {\em Member Levels} calculated by the NewsTrust staff based on  community engagement, time in the community, other users' feedback on reviews, profile transparency, and manual validation.
We use these member levels to categorize users as {\em experienced} or {\em inexperienced}. This is treated as the ground truth for assessing the prediction and ranking quality of our model and the baseline ``user at learned rate'' model~\cite{mcauleyWWW2013}.
Table~\ref{tab:ndcgUsers} shows the $F_1$ scores of these two competitors.
We also computed the \emph{Normalized Discounted Cumulative Gain (NDCG)} \cite{Jarvelin:TOIS2002} 
%Kalervo Jarvelin, Jaana Kekalainen: Cumulated gain-based evaluation of IR 
%techniques. ACM Transactions on Information Systems 20(4), 422–446 (2002)
for the ranked lists of users generated by the two models. NDCG gives geometrically decreasing weights to predictions at various positions of ranked list:

{
$NDCG_p = \frac{DCG_p}{IDCG_p}$ where
$DCG_p = rel_1 + \sum_{i=2}^p \frac{rel_i}{\log_2 i}$
}

Here, $rel_i$ is the relevance ($0$ or $1$) of a result at position $i$. 
%DCG penalizes relevant items (\emph{experienced users}) appearing lower in 
%the rank list, where the graded relevance score is reduced logarithmically 
%proportional to the position of the result. 
%As the length of lists may vary for different queries, DCG scores are 
%normalized using the ideal score, IDCG where the results of a rank list are 
%sorted by relevance giving the maximum possible DCG score.

As Table~\ref{tab:ndcgUsers} shows, our model clearly outperforms the baseline model on both $F_1$ and $NDCG$.

==> main/introduction/abstract.tex <==

\chapter*{Abstract}

\section*{}

One of the major hurdles preventing the full exploitation of information from online communities is the widespread concern regarding the quality and credibility of user-contributed content. Prior works in this domain operate on a static snapshot of the community, making strong assumptions about the structure of the data (e.g., relational tables), or consider only shallow features for text classification.\\

To address the above limitations, we propose probabilistic graphical models that can leverage the joint interplay between multiple factors in online communities --- like user interactions, community dynamics, and textual content --- to automatically assess the credibility of user-contributed online content, and the expertise of users and their evolution with user-interpretable explanation. To this end, we devise new models based on Conditional Random Fields for different settings like incorporating partial expert knowledge for semi-supervised learning, and handling discrete labels as well as numeric data for fine-grained analysis. This enables applications such as extracting reliable side-effects of drugs from user-contributed posts in healthforums, and identifying credible content in news communities.\\

Online communities are dynamic, as users join and leave, adapt to evolving trends, and mature over time. To capture this dynamics, we propose generative models based on Hidden Markov Model, Latent Dirichlet Allocation, and Brownian Motion to trace the continuous evolution of user expertise and their language model over time. This allows us to identify expert users and credible content jointly over time, improving state-of-the-art recommender systems by explicitly considering the maturity of users. This enables applications such as identifying useful product reviews, and detecting fake and anomalous reviews with {limited} information.

==> tail/bibliography.tex <==
@inproceedings{fogg2003,
	author    = {B. J. Fogg},
	title     = {Prominence-interpretation theory: explaining how people assess credibility
	online},
	booktitle = {{CHI}},
	year = {2003}
}

@inproceedings{castillo2011,
	author    = {Carlos Castillo and
	Marcelo Mendoza and
	Barbara Poblete},
	title     = {Information credibility on twitter},
	booktitle = {
	{WWW}},
	year = {2011}
}

@article{DBLP:journals/intr/CastilloMP13,
	author    = {Carlos Castillo and
	Marcelo Mendoza and
	Barbara Poblete},
	title     = {Predicting information credibility in time-sensitive social media},
	journal   = {Internet Research},
	year      = {2013},
	volume    = {23},
	number    = {5},
}

@inproceedings{agupta2012,
	author = {Gupta, Aditi and Kumaraguru, Ponnurangam},
	title = {Credibility Ranking of Tweets During High Impact Events},
	booktitle = {PSOSM},
	year = {2012}}

@inproceedings{canini2011,
	author    = {Kevin Robert Canini and
	Bongwon Suh and
	Peter Pirolli},
	title     = {Finding Credible Information Sources in Social Networks Based on Content
	and Social Structure},
	booktitle = {PASSAT},
	year = {2011}
}

@inproceedings{kang2012,
	author = {Kang, Byungkyu and O'Donovan, John and H\"{o}llerer, Tobias},
	title = {Modeling Topic Specific Credibility on Twitter},
	booktitle = {IUI},
	year = {2012}
}

@inproceedings{vg2011,
	author = {Vydiswaran, V.G. Vinod and Zhai, ChengXiang and Roth, Dan},
	title = {Content-driven Trust Propagation Framework},
	booktitle = {KDD},
	year = {2011}
}


@misc{nber,
	author = {Nber.org},
	title = {Media Bias and Voting},
	howpublished = {{\scriptsize http://www.nber.org/digest/oct06/w12169.html}},
	note = {{\footnotesize Accessed: 2015-05-07}
}
}

@misc{pp2,
	author = {Meta.stackexchange.com},
	title = {The problem with reputation: does high reputation attract too many upvotes?},
	howpublished = {{\scriptsize http://meta.stackexchange.com/questions/515/the-problem-with-reputation-does-high-reputation-attract-too-many-upvotes}},
	note = {{\footnotesize Accessed: 2015-04-07}}
}

@misc{sloanreview,
	author = {Sloanreview.mit.edu},
	title = {The Problem With Online Ratings},
	howpublished = {{\scriptsize http://sloanreview.mit.edu/article/the-problem-with-online-ratings-2/ }},
	note = {{\footnotesize Accessed: 2015-05-07}}
}

@misc{pp4,		
	author = {Rhetorica.net},
	title = {Media / Political Bias},
	howpublished = {{\scriptsize http://rhetorica.net/bias.htm}},
	note = {{\footnotesize Accessed: 2015-04-07}}
}

@misc{global-research,
	author = {Globalresearch.ca},
	title = {Information, Disinformation and the Credibility Crisis. Where is the Truth in Today's News Reporting?},
	howpublished = {{\scriptsize http://www.globalresearch.ca/information-disinformation-and-the-credibility-crisis-where-is-the-truth-in-todays-news-reporting/5373876}},
	note = {{\footnotesize Accessed: 2015-04-07}}
}


@misc{pp6,
	author = {Poynter.org},
	title = {Studying Newspapers in a Time of Change},
	howpublished = {{\scriptsize http://www.poynter.org/uncategorized/99225/studying-newspapers-in-a-time-of-change/}},
	note = {{\footnotesize Accessed: 2015-04-07}}
}

@misc{pp7,
	author = {Liberty.uoregon.edu},
	title = {Critical Evaluation of Information Sources},
	howpublished = {{\scriptsize http://library.uoregon.edu/guides/findarticles/credibility.html}},
	note = {{\footnotesize Accessed: 2015-04-07}}
}

@misc{gallop,
	author = {Gallup.com},
	title = {Americans' Confidence in Newspapers Continues to Erode},
	howpublished = {{\scriptsize http://www.gallup.com/poll/163097/americans-confidence- newspapers-continues-erode.aspx}},
	note = {{\footnotesize Accessed: 2015-05-07}},
}

@book{chomsky1988,
	author = {Herman, Edward S. and Chomsky, Noam},
	title = {{Manufacturing consent : the political economy of the mass media}},
	year = {1988}
}

@article{dellavigna2007,
	author = {DellaVigna, Stefano and Kaplan, Ethan},
	journal = {Quarterly Journal of Economics},
	title = {The Fox News Effect: Media Bias and Voting},
	volume = {122},
	year = {2007}
}

@article{Muchnik13,
	author = {Muchnik, Lev and Aral, Sinan and Taylor, Sean J.},
	journal = {Science},
	number = {6146},
	title = {{Social Influence Bias: A Randomized Experiment}},
	volume = {341},
	year = {2013}
}

@inproceedings{Garbett:2014:FRP:2556288.2557114,
	author = {Garbett, Andrew Thomas and Comber, Rob and Egglestone, Paul and Glancy, Maxine and Olivier, Patrick},
	title = {Finding "Real People": Trust and Diversity in the Interface Between Professional and Citizen Journalists},
	booktitle = {CHI},
	year = {2014}
}

@inproceedings{fang2014,
	author = {Fang, Hui and Zhang, Jie and Magnenat Thalmann, Nadia},
	title = {Subjectivity Grouping: Learning from Users' Rating Behavior},
	booktitle = {AAMAS},
	year = {2014}
}

@inproceedings{Kakol:2013:SBW:2487788.2488133,
	author = {Kakol, Michal and Jankowski-Lorek, Michal and Abramczuk, Katarzyna and Wierzbicki, Adam and Catasta, Michele},
	title = {On the Subjectivity and Bias of Web Content Credibility Evaluations},
	booktitle = {WWW Companion},
	year = {2013}
}

@book{paul2006,
	author = {Paul, R., and Elder, L.},
	publisher = {Foundation for Critical Thinking: Tomles, CA.},
	title = {{How to detect media bias and propaganda}},
	year = {2006}
}

@inproceedings{lampe2007,
  author = {Lampe, Cliff and Garrett, R. Kelly},
  booktitle = {HICSS},
  title = {It's All News to Me: The Effect of Instruments on Ratings Provision.},
  year = {2007}
}

@inproceedings{mukherjee2014,
 author = {Mukherjee, Subhabrata and Weikum, Gerhard and Danescu-Niculescu-Mizil, Cristian},
 title = {People on Drugs: Credibility of User Statements in Health Communities},
 series = {KDD},
 year = {2014}
}


@inproceedings{greene2009,
 author = {Greene, Stephan and Resnik, Philip},
 title = {More Than Words: Syntactic Packaging and Implicit Sentiment},
 booktitle = {NAACL},
 year = {2009}
}

@inproceedings{recasens2013,
  author={Marta Recasens and Cristian Danescu-Niculescu-Mizil and Dan Jurafsky},
  title={Linguistic Models for Analyzing and Detecting Biased Language},
  booktitle={ACL},
  year = {2013}
}

@inproceedings{wiebe2005,
 author = {Wiebe, Janyce and Riloff, Ellen},
 title = {Creating Subjective and Objective Sentence Classifiers from Unannotated Texts},
 booktitle = {CICLing},
 year = {2005}
}

@inproceedings{lin2011,
  author    = {Chenghua Lin and
               Yulan He and
               Richard Everson},
  title     = {Sentence Subjectivity Detection with Weakly-Supervised Learning},
  booktitle = {{IJCNLP}},
  year = {2011}
}

@inproceedings{drucker1996,
  author    = {Harris Drucker and
               Christopher J. C. Burges and
               Linda Kaufman and
               Alex J. Smola and
               Vladimir Vapnik},
  title     = {Support Vector Regression Machines},
  booktitle = {NIPS},
  year = {1996}
}

@article{flanagin2000,
    author = {Flanagin, A. J. and Metzger, M. J.},
    journal = {Journalism and Mass Communication Quarterly},
    number = {3},
    title = {{Perceptions of Internet information credibility}},
    volume = {77},
    year = {2000}
}

@article{johnson2007,
    author = {Johnson, Thomas J. and Kaye, Barbara K. and Bichard, Shannon L. and Wong, W. Joann},
    journal = {Journal of Computer-Mediated Communication},
    keywords = {blogs, credibility, news},
    number = {1},
    title = {{Every blog has its day: Politically-interested Internet users' perceptions of blog credibility.}},
    volume = {13},
    year = {2007}
}

@article{howard2011,
author = {Philip N. Howard and Aiden Duffy and Deen Freelon and Muzammil Hussain and Will Mari and Marwa Mazaid},
title = {Opening Closed Regimes: What Was the Role of Social Media During the Arab Spring?},
year = {2011},
}

@misc{boston,
	author = {Nytimes.com},
	title = {Should Reddit Be Blamed for the Spreading of a Smear?},
	howpublished = {{\scriptsize http://www.nytimes.com/2013/07/28/magazine/should-reddit-be- blamed-for-the-spreading-of-a-smear.html}},
	note = {{\small Accessed: 2015-05-07}},
}

@article{wemedia, 
title={We Media: How Audiences are Shaping the Future of News and Information}, 
url={{\scriptsize http://www.hypergene.net/wemedia/weblog.php}}, 
author={Bowman Shayne and Willis Chris}, 
year={2003}
}


@inproceedings{garbett2014,
 author = {Garbett, Andrew Thomas and Comber, Rob and Egglestone, Paul and Glancy, Maxine and Olivier, Patrick},
 title = {Finding "Real People": Trust and Diversity in the Interface Between Professional and Citizen Journalists},
 booktitle = {CHI},
 year = {2014}
}

@article{lewis2010,
  title={Thinking about citizen journalism: The philosophical and practical challenges of user-generated content for community newspapers},
  author={Lewis, Seth C and Kaufhold, Kelly and Lasorsa, Dominic L},
  journal={Journalism Practice},
  volume={4},
  number={2},
  year={2010},
}

@article{allan2007,
  title={Citizen Journalism and the Rise of `Mass Self-Communication': Reporting the London Bombings.},
  author={Stuart, Allan},
  journal={Global Media},
  volume={1},
  number={1},
  year={2007},
}

@article{blei2003,
 author = {Blei, David M. and Ng, Andrew Y. and Jordan, Michael I.},
 title = {Latent Dirichlet Allocation},
 journal = {J. Mach. Learn. Res.},
 volume = {3},
 year = {2003},
}

@inproceedings{mukherjee2014JAST,
author = {Subhabrata Mukherjee and Gaurab Basu and Sachindra Joshi},
title = {Joint Author Sentiment Topic Model},
booktitle = {SDM},
year = {2014}
}

@inproceedings{mukherjee2013WWW,
  author    = {Subhabrata Mukherjee and
               Gaurab Basu and
               Sachindra Joshi},
  title     = {Incorporating author preference in sentiment rating prediction of
               reviews},
  booktitle = {{WWW}},
  year = {2013}
}

@ARTICLE{einhorn1977,
    author = {Hillel J. Einhorn and Robin M. Hogarth and Eric Klempner},
    title = {Quality of group judgment},
    journal = {Psychological Bulletin},
    year = {1977},
}

@inproceedings{mcauley2013,
  author = {J. J. McAuley and J. Leskovec},
  title = {From amateurs to connoisseurs: modeling the evolution of user expertise through online reviews},
  booktitle = {WWW},
  year = {2013}
}

@inproceedings{rosenzviUAI2004,
 author = {Rosen-Zvi, Michal and Griffiths, Thomas and Steyvers, Mark and Smyth, Padhraic},
 title = {The Author-topic Model for Authors and Documents},
 series = {UAI},
 year = {2004},
}

@inproceedings{radosavljevicECAI2010,
 author = {Radosavljevic, Vladan and Vucetic, Slobodan and Obradovic, Zoran},
 title = {Continuous Conditional Random Fields for Regression in Remote Sensing},
 series = {ECAI},
 year = {2010},
}

@inproceedings{qinNIPS2008,
  author    = {Tao Qin and
               Tie{-}Yan Liu and
               Xu{-}Dong Zhang and
               De{-}Sheng Wang and
               Hang Li},
  title     = {Global Ranking Using Continuous Conditional Random Fields},
  series = {NIPS},
  year      = {2008},
}

@inproceedings{korenKDD2008,
 author = {Koren, Yehuda},
 title = {Factorization Meets the Neighborhood: A Multifaceted Collaborative Filtering Model},
 series = {KDD},
 year = {2008},
}

@inproceedings{mcauleyrecsys2013,
 author = {McAuley, Julian and Leskovec, Jure},
 title = {Hidden Factors and Hidden Topics: Understanding Rating Dimensions with Review Text},
 series = {RecSys},
 year = {2013},
}

@inproceedings{linCIKM2009,
 author = {Lin, Chenghua and He, Yulan},
 title = {Joint Sentiment/Topic Model for Sentiment Analysis},
 series = {CIKM},
 year = {2009},
}

@inproceedings{wang2011,
 author = {Wang et al., Hongning},
 title = {Latent aspect rating analysis without aspect keyword supervision},
 series = {KDD},
 year = {2011},
}

@article{West-etal:2014,
  Author = {West, Robert  and  Paskov, Hristo S. and  Leskovec, Jure  and  Potts, Christopher},
  Title = {Exploiting Social Network Structure for Person-to-Person Sentiment Analysis},
  Journal = {TACL},
  Volume = {2},
  Number = {2},
  Year = {2014}}
@article{Jarvelin:TOIS2002,
  author    = {Kalervo J{\"{a}}rvelin and
               Jaana Kek{\"{a}}l{\"{a}}inen},
  title     = {Cumulated gain-based evaluation of {IR} techniques},
  journal   = {{ACM} Trans. Inf. Syst.},
  volume    = {20},
  number    = {4},
  year      = {2002},
}

@inproceedings{Gunnemann2014,
 author = {G\"{u}nnemann, Stephan and G\"{u}nnemann, Nikou and Faloutsos, Christos},
 title = {Detecting Anomalies in Dynamic Rating Data: A Robust Probabilistic Model for Rating Evolution},
 series = {KDD},
 year = {2014},
}

@inproceedings{DanescuWWW2013,
  author={Cristian Danescu-Niculescu-Mizil and Robert West and Dan Jurafsky
  and Jure Leskovec and Christopher Potts},
  title={No country for old members: {User} lifecycle and linguistic change in
  online communities},
  series={WWW},
  year={2013}
}

@inproceedings{VZRPCIKM12,
	author = {V.G.Vinod Vydiswaran and others},
	title = {{BiasTrust: Teaching biased users about controversial topics}},
	series = {CIKM},
	year = {2012}
}

@inproceedings{tadas14,
  author    = {Baltrusaitis Tadas and
               Peter Robinson and
               Louis{-}Philippe Morency},
  title     = {Continuous Conditional Neural Fields for Structured Regression},
  booktitle = {ECCV},
  year      = {2014},
}

%---------------------------------------------------------------------------------------------%

@article{YaliangLi:SIGKDD2015,
  author    = {Yaliang Li and
               Jing Gao and
               Chuishi Meng and
               Qi Li and
               Lu Su and
               Bo Zhao and
               Wei Fan and
               Jiawei Han},
  title     = {A Survey on Truth Discovery},
  journal   = {{SIGKDD} Explorations},
  volume    = {17},
  number    = {2},
  pages     = {1--16},
  year      = {2015},
  url       = {http://doi.acm.org/10.1145/2897350.2897352},
  doi       = {10.1145/2897350.2897352},
  timestamp = {Thu, 17 Mar 2016 09:20:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/sigkdd/LiGMLSZFH15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Dong:2015:KTE:2777598.2777603,
	author = {Dong, Xin Luna and Gabrilovich, Evgeniy and others},
	title = {Knowledge-based Trust: Estimating the Trustworthiness of Web Sources},
	journal = {Proc. VLDB Endow.},
	issue_date = {May 2015},
	volume = {8},
	number = {9},
	month = may,
	year = {2015},
	issn = {2150-8097},
	pages = {938--949},
	numpages = {12},
	url = {http://dx.doi.org/10.14778/2777598.2777603},
	doi = {10.14778/2777598.2777603},
	acmid = {2777603},
	publisher = {VLDB Endowment},
} 

@article{DBLP:journals/pvldb/LiDLMS12,
	author    = {Xian Li and
	Xin Luna Dong and
	Kenneth Lyons and
	Weiyi Meng and
	Divesh Srivastava},
	title     = {Truth Finding on the Deep Web: Is the Problem Solved?},
	journal   = {{PVLDB}},
	volume    = {6},
	number    = {2},
	pages     = {97--108},
	year      = {2012},
	url       = {http://www.vldb.org/pvldb/vol6/p97-li.pdf},
	timestamp = {Wed, 04 Sep 2013 08:28:44 +0200},
	biburl    = {http://dblp.uni-trier.de/rec/bib/journals/pvldb/LiDLMS12},
	bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Li:2011:TVT:2004686.2005589,
	author = {Li, Xian and Meng, Weiyi and Yu, Clement},
	title = {T-verifier: Verifying Truthfulness of Fact Statements},
	booktitle = {ICDE 2011},
	url = {http://dx.doi.org/10.1109/ICDE.2011.5767859},
	doi = {10.1109/ICDE.2011.5767859},
	acmid = {2005589},
} 

 @inproceedings{Li:2015:DET:2783258.2783277,
 	author = {Li, Yaliang and Li, Qi and Gao, Jing and Su, Lu and Zhao, Bo and Fan, Wei and Han, Jiawei},
 	title = {On the Discovery of Evolving Truth},
 	booktitle = {KDD 2015},
 	location = {Sydney, NSW, Australia},
 	numpages = {10},
 	url = {http://doi.acm.org/10.1145/2783258.2783277},
 	doi = {10.1145/2783258.2783277},
 	acmid = {2783277},
 	keywords = {dynamic data, source reliability, truth discovery},
 } 
 
 

